Unsupervised Online Video Object Segmentation with Motion Property Understanding

Unsupervised video object segmentation aims to automatically segment moving objects over an unconstrained video without any user annotation. So far, only few unsupervised online methods have been reported in literature and their performance is still far from satisfactory, because the complementary information from future frames cannot be processed under online setting. To solve this challenging problem, in this paper, we propose a novel Unsupervised Online Video Object Segmentation (UOVOS) framework by construing the motion property to mean moving in concurrence with a generic object for segmented regions. By incorporating salient motion detection and object proposal, a pixel-wise fusion strategy is developed to effectively remove detection noise such as dynamic background and stationary objects. Furthermore, by leveraging the obtained segmentation from immediately preceding frames, a forward propagation algorithm is employed to deal with unreliable motion detection and object proposals. Experimental results on several benchmark datasets demonstrate the efficacy of the proposed method. Compared to the state-of-the-art unsupervised online segmentation algorithms, the proposed method achieves an absolute gain of 6.2%. Moreover, our method achieves better performance than the best unsupervised offline algorithm on the DAVIS-2016 benchmark dataset. Our code is available on the project website: https://github.com/visiontao/uovos.

==> sec_acknowledgment.tex <==
\section*{Acknowledgment}
\label{sec:acknowledgement}

This research is supported by the National Research Foundation, Prime Minister's Office, Singapore under its Strategic Capability Research Centres Funding Initiative. This research is also supported by National Natural Science Foundation of China 61571362 and Natural Science Basic Research Plan in Shaanxi Province of China (Program No. 2018JM6015).



==> sec_motion.tex <==
\section{Background of Geometry-based Models}
\label{sec:motion}

Given a set of corresponding points in two image views,
the point coordinates between the two images can be mapped by a geometric model.
Geometric models include homography transform and fundamental matrix \cite{Hartley2004},
which are widely used in many visual tasks \cite{Hartley2004},
such as camera motion estimation, image stitching, panoramic mosaic and 3D reconstruction. 

For moving object segmentation in moving camera environments, 
the early works often estimate a homography transform or fundamental matrix to model the unknown camera motion.
Given a set of corresponding pixels between two consecutive frames,
a global homography transform or fundamental matrix model can be estimated by the RANSAC algorithm \cite{Hartley2004}.
Then, 
based on the assumption that background pixels are dominant,
then the foreground/background pixels are predicted as outliers/inliers \cite{ICCV2009_Sheikh,ECCV2014_Zamalieva,TOG2016_Zhang,CVPR2014_Jung,CVPR2007_Bugeau}.

Since the structure of real world is complex,
accurate modeling of unknown camera motion \cite{Hartley2004} with fundamental matrix and homography is a challenging task.
When the camera moves,
the scene near to the camera has larger pixel displacement than those far away from camera.
The advantage of fundamental matrix is that it is not sensitive to different scene depths.
However, fundamental matrix requires camera translation to create parallax.
and it is only valid for nonplanar and rigid scenes, which limit its application in general conditions.
In contrast, homography transform is only valid for planar scenes, 
and it is not accurate when strong parallax exists.
but it can be used for non-rigid scene and object. 
Since a single model is not accurate enough to represent the real world,
some methods try a multi-model fitting strategy \cite{CVPR2014_Luca} for accurate scene representation.
Luca \etal use multiple fundamental matrices to describe each rigid object and multiple homographies to fit each planar.
Compared to single model fitting method,
although multi-model is more accurate in describing the real world,
but its computation cost is very high \cite{CVPR2014_Luca}.

Although there are some constraints in the geometric model,
it still provides important foreground/background information. 
Considering both computation cost and model constraints,
we adopt the global homography to model the camera motion and background as in \cite{ICCV2009_Sheikh,ECCV2014_Zamalieva,TOG2016_Zhang},
and we use the geometric model fitting error to identify the foreground/background region in dynamic video scene.
In addition,
due to lack of prior knowledge about the foreground/background ratio of the whole scene, 
geometric model estimation is a chicken-\&-egg problem,
and the moving foreground segmentation cannot be simply distinguished as outliers \cite{Hartley2004} by a given threshold.
Therefore, instead of geometry-based models alone,
we incorporate the homography model into the salient motion extraction for improved moving object segmentation.



